AttacKG: Constructing Technique Knowledge Graph from Cyber Threat Intelligence Reports

Cyber attacks are becoming more sophisticated and diverse, making detection increasingly challenging. To combat these attacks, security practitioners actively summarize and exchange their knowledge about attacks across organizations in the form of cyber threat intelligence (CTI) reports. However, as CTI reports written in natural language texts are not structured for automatic analysis, the report usage requires tedious manual efforts of cyber threat intelligence recovery. Additionally, individual reports typically cover only a limited aspect of attack patterns (techniques) and thus are insufficient to provide a comprehensive view of attacks with multiple variants. To take advantage of threat intelligence delivered by CTI reports, we propose AttacKG to automatically extract structured attack behavior graphs from CTI reports and identify the adopted attack techniques. We then aggregate cyber threat intelligence across reports to collect different aspects of techniques and enhance attack behavior graphs into technique knowledge graphs (TKGs). In our evaluation against 1,515 real-world CTI reports from diverse intelligence sources, AttacKG effectively identifies 28,262 attack techniques with 8,393 unique Indicators of Compromises (IoCs). To further verify the accuracy of AttacKG in extracting threat intelligence, we run AttacKG on 16 manually labeled CTI reports. Empirical results show that AttacKG accurately identifies attack-relevant entities, dependencies, and techniques with F1-scores of 0.887, 0.896, and 0.789, which outperforms the state-of-the-art approaches Extractor and TTPDrill. Moreover, the unique technique-level intelligence will directly benefit downstream security tasks that rely on technique specifications, e.g., APT detection and cyber attack reconstruction.

==> 8_Related_Work.tex <==
\subsection{Related Work}
\label{sec:relatedworks}

\subsubsection{Threat Intelligence Extraction.}
Cyber threat intelligence (CTI) plays a vital role in security warfare to keep up with the rapidly evolving landscape of cyber attacks~\cite{mu2018understanding,gao2021system}.
To facilitate CTI knowledge exchange and management, the security community has standardized open formats (e.g., OpenIoC~\cite{OpenIOC}, STIX~\cite{STIX}, and CybOX~\cite{CybOX}) to describe Indicators of Compromises (IoCs).
Though structured and machine-readable, such intelligence lacks semantic information about how entities/IoCs interact to form the kill chain. 
While in this paper, we try to fulfill this semantic gap with technique-level knowledge aggregated from multiple CTI reports.

While such CTI reports provide detailed contexts about an attack (e.g., the sequence of adversarial actions), manually extracting attack-relevant information from uninstructed texts is labor-intensive and error-prone, hindering CTI's practice applications.
Based on the observation that IoCs often share similar context terms, iACE~\cite{Liao} presents a graph mining technique to collect IoCs available in tens of thousands of security articles.
ChainSmith~\cite{Zhu2018} further makes use of neural networks to classify IoCs into different attack campaign stages (e.g., baiting and C\&C).
TTPDrill~\cite{Husari2017} derives threat actions from Symantec reports and maps them to attack patterns (e.g., techniques in MITRE ATT\&CK~\cite{mitre}) pre-defined as ontology.
EXTRACTOR~\cite{Satvat2021} and ThreatRaptor~\cite{gao} customize NLP techniques to model attacks behaviors in texts as provenance graphs.
Similar to prior studies, the large body of \sysname is to automate knowledge extraction from CTI.
Nevertheless, \sysname distinguishes from these works in the sense that it identifies TTPs and constructs a technique knowledge graph (TKG) to summarize technique-level knowledge in CTI reports.

\subsubsection{Threat Detection with Cyber Intelligence.}
Recent advancements of causality analysis in provenance graph~\cite{king2003backtracking,king2005enriching,pohly2012hi,bates2015trustworthy} have enabled security investigators to detect cyber attacks with multiple stages.
However, audit logs monitor general-purpose system activities and thus lack the knowledge of high-level behaviors~\cite{zengwatson}.
In most cases, analysts act as the backbone in SOCs (security operations center) to correlate various attack stages through reviewing numerous system logs~\cite{vanede2020deepcase}.
Unfortunately, as the volume of audit data is typically overwhelming even after reducing noisy logs irrelevant to attacks~\cite{lee2013loggc,xu2016high,liu2018towards,tang2018nodemerge,michael2020forensic,hassan2020we}, it is infeasible to manually analyze cyber threats directly based on audit logs~\cite{gao2018aiql,gao2018saql}.

CTI has proved to be valuable information in navigating audit logs and pinpointing behaviors associated with known attacks~\cite{MomeniMilajerdi2019,Milajerdi2019,hossain2020combating,Hassan2020,gao}.
For example, RapSheet~\cite{Hassan2020} matches audit logs against a TTP knowledge base from MITRE and correlates TTPs in logs and constructs a TPG (tactic provenance graph) to recover \textit{kill chains} in APT campaigns.
We envision that the deployment of \sysname can enhance any detectors that rely on TTP heuristics by providing a fully automated solution for constructing TKGs from CTI reports.


==> A1_Attack_Samples.tex <==
\section{Manually Labeled CTI Report Samples}
\label{appendix:samples}

\begin{figure*}[t]
    \centering
    \includegraphics[width=7in]{Image/Evaluation_sample/Evaluation_sample_1.pdf}
    \vspace{-0.2in}
    \caption{TC\_Firefox DNS Drakon APT.}
    \label{fig:sample_1}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=7in]{Image/Evaluation_sample/Evaluation_sample_2.pdf}
    \vspace{-0.2in}
    \caption{TC\_Firefox Drakon APT Elevate Copykatz.}
    \label{fig:sample_2}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=7in]{Image/Evaluation_sample/Evaluation_sample_3.pdf}
    \vspace{-0.2in}
    \caption{TC\_Firefox BITS Micro APT.}
    \label{fig:sample_3}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=7in]{Image/Evaluation_sample/Evaluation_sample_4.pdf}
    \vspace{-0.2in}
    \caption{TC\_SSH BinFmt-Elevate.}
    \label{fig:sample_4}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=7in]{Image/Evaluation_sample/Evaluation_sample_5.pdf}
    \vspace{-0.2in}
    \caption{TC\_Nginx Drakon APT.}
    \label{fig:sample_5}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=7in]{Image/Evaluation_sample/Evaluation_sample_6.pdf}
    \vspace{-0.2in}
    \caption{Frankenstein Campaign.}
    \label{fig:sample_6}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=7in]{Image/Evaluation_sample/Evaluation_sample_7.pdf}
    \vspace{-0.2in}
    \caption{OceanLotus(APT32) Campaign.}
    \label{fig:sample_7}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=7in]{Image/Evaluation_sample/Evaluation_sample_8.pdf}
    \vspace{-0.2in}
    \caption{Cobalt Campaign.}
    \label{fig:sample_8}
\end{figure*}

==> A2_Attack_variants.tex <==
% \section{Attack Variants Extracted from CTI Reports}


==> A3_Comparsion_of_OSCTI <==
% \section{Comparsion of Our OSCTI Content and Existing Industry Works}

==> Archive/4_Technique_Kowledge_Graph.tex <==
\section{Technique Knowledge Graph}
\label{sec:tkg}

\subsection{TKG design}

The TKG should take a hierarchical (two-layer) design, namely, system entity (and action) level and TTP level. On system entity level, the TKG looks just like many sub-graphs(TPG) of Provenance Graph.  Every sub-graph represents a TTP and make up the TTP-level TKG. Every TTP node should have one or more inputs and outputs. And we can use these inputs and outputs connect TTPs.


\subsubsection{Layer 1: kill chain layer}

\subsubsection{Layer 2: TTP representation layer}

\subsection{Initing the TKG – The Workflow:
}

\begin{figure}
    \centering
    \includegraphics[width=3.3in]{Image/architecture.png}
    \caption{Attack Knowledge Graph Building Process.}
    \label{fig:architecture}
\end{figure}

\subsubsection{NLP-based CTI report parsing: the input is CTI reports and description for all the TTPs (mitre attack)}
\label{sub_sec:nlp_parser}

\begin{figure}
    \centering
    \includegraphics[width=3.3in]{Image/nlp_architecture.png}
    \caption{NLP-based Report Parsiing Process.}
    \label{fig:nlp_architecture}
\end{figure}

\ToDo{S2-0. Preprocess}

\ToDo{S2-1,2. NLP-based TTP extraction}

\ToDo{S2-3. Relation extraction}

\ToDo{S2-4. Co-reference resolution}

\ToDo{S2-5. Attack graph reconstruction for each TTP segment}

\subsubsection{TKG initialization-update-loop: the input is subgraphs representing TTPs}
\label{sub_sec:TKG_update}


\ToDo{1 Find similar subgraphs in TKG according to TTP, input/output, IoCs, subgraph structure.}

\ToDo{2 If not match, add subgraphs to the TKG; If match, find the difference and try to abstract a more general model to match both graph.}

\ToDo{3 Try to connect the new TTP with other TTPs according to the inputs and outputs.}

\subsection{TKG matching}
\label{sub_sec:matching}

\ToDo{Speed up the matching process by key nodes matching.}


==> Archive/5_TKG_Case_Study.tex <==
\section{TKG Application}
\label{sec:applicaiton}

\subsection{TKG can help with the detection of threat}

\subsection{TKG can help with the understanding of threat reports}

